The Creativity of Text-to-Image Generation

Text-guided synthesis of images has made a giant leap towards becoming a mainstream phenomenon. With text-to-image generation systems, anybody can create digital images and artworks. This provokes the question of whether text-to-image generation is creative. This paper expounds on the nature of human creativity involved in text-to-image art (so-called "AI art") with a specific focus on the practice of prompt engineering. The paper argues that the current product-centered view of creativity falls short in the context of text-to-image generation. A case exemplifying this shortcoming is provided and the importance of online communities for the creative ecosystem of text-to-image art is highlighted. The paper provides a high-level summary of this online ecosystem drawing on Rhodes' conceptual four P model of creativity. Challenges for evaluating the creativity of text-to-image generation and opportunities for research on text-to-image generation in the field of Human-Computer Interaction (HCI) are discussed.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> MindTrek22 Creativity of Text-to-Image Generation/FIGURE1.tex <==
%TC:ignore
\newlength{\bigimgwidth}%
\setlength{\bigimgwidth}{.4\textwidth}%
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!ht]
\centering
\begin{tabularx}{\textwidth}{YY}%
%
    \includegraphics[width=\bigimgwidth]{figures/lyrics/whatif2.jpg}%
 &%
    \includegraphics[width=\bigimgwidth]{figures/lyrics/baba.jpg}%
\\%
    % \small
    \textit{What if everything around you isn't quite as it seems What if all the world you used to know Is an elaborate dream. Painting by Haralampi Oroschakoff, trending on wikiart}\newline%
    (lyrics from the song `Right Where It Belongs' by Nine Inch Nails)%
&
    % \small
    \textit{How long will this take, baba? And how long have we been sleeping? Do you see me hanging on to every word you say? How soon will I be holy? How much will this cost, guru? How much longer till you completely absolve me?}\newline%
    (lyrics from the song `Baba' by Alanis Morissette)%
\vspace{1em}
\\
    \includegraphics[width=\bigimgwidth]{figures/lyrics/mirror.jpg}
 &
    \includegraphics[width=\bigimgwidth]{figures/lyrics/FQiuAElWQAAoG97.jpg}
\\
    % \small
        \textit{When I see the man in the mirror I see an animal clearer}\newline%
        (lyrics from the song `Hot' by CunninLynguists)
&
    % \small
        \textit{Soaked in soul, he swims in my eyes by the bed}\newline%
        (lyrics from the song `Wake Up Alone' by Amy Winehouse)
\end{tabularx}%
  \caption{Examples of images generated from parts of music lyrics with Midjourney's CLIP guided diffusion \cite{midjourney}.
  Figure a) demonstrates the use of additional prompt modifiers.
  Figures b) and c) were created without prompt modifiers.}%
  \Description{Examples of images generated from parts of music lyrics.}%
  \label{fig:examples1}%
\end{figure*}%
%TC:endignore

==> MindTrek22 Creativity of Text-to-Image Generation/FIGURE2.tex <==

% ------------
%TC:ignore
\newlength{\imagewidth}%
\setlength{\imagewidth}{.18\textwidth}%
% ------------
\newcommand{\mytd}[1]{\small{\multicolumn{1}{c}{#1}}}
% \newcommand{\mytdbf}[1]{\textbf{\multicolumn{2}{c}{#1}}}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!ht]
\centering
\begin{tabularx}{\textwidth}{YYYYY}
    \multicolumn{2}{c}{\textbf{Single characters}}
       &
    \textbf{Single words}
       &
    \textbf{Movie quotes}
       &
    \textbf{Emojis}
\vspace{.5em}
\\
    \includegraphics[width=\imagewidth]{figures/characters/pyramid.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/characters/O.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/words/limitless-2.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/movies/ill-be-back.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/emojis/grinning-face.jpg}
    \\
        a) $\Delta$% Δ
       &
        b) O
       &
        c) \textit{limitless}
       &
        d) \textit{I'll be back}
       &
        e) % \emoji{grinning-face}
        \includegraphics[width=11pt,height=11pt,align=c]{figures/emojis/google-grinning-face_1f600.png}
\vspace{.5em}
\\
      \includegraphics[width=\imagewidth]{figures/characters/infinity-1.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/characters/V.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/words/daydreaming.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/movies/Viva_los_bio_dome.jpg}
       &
    \includegraphics[width=\imagewidth]{figures/emojis/smiling-face-with-sunglasses.jpg}
    \\
        f) $\infty$
       &
        g)  V
       & 
        h) \textit{daydreaming}
       & 
        i) \textit{viva los} [sic]
           \newline
           \textit{bio dome}
       & 
        j)  % \emoji{smiling-face-with-sunglasses}
        \includegraphics[width=11pt,height=11pt,align=c]{figures/emojis/google-smiling-face-with-sunglasses_1f60e.png}%
\\%
\end{tabularx}%
  \caption{Examples of images generated with Midjourney CLIP guided diffusion without style modifiers~\cite{midjourney}.}%
  \Description{Examples of images generated with Midjourney CLIP guided diffusion without style modifiers.}%
  \label{fig:examples2}%
\end{figure*}%
%TC:endignore


==> MindTrek22 Creativity of Text-to-Image Generation/FIGURE3.tex <==

% ------------
%TC:ignore
\newlength{\imagewidthcuration}
\setlength{\imagewidthcuration}{.23\textwidth}
%TC:endignore
% ------------

%TC:ignore
\begin{figure*}[!ht]
\centering
\begin{tabular}{ccccc}
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/0.jpg}
       &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/25.jpg}
       &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/50.jpg}
       &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/75.jpg}
    \\
        Step 0
       &
        Step 25
       &
        Step 50
       &
        Step 75
    \\
\addlinespace[1ex]

    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/100.jpg}
       &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/125.jpg}
        &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/150.jpg}
        &
    \includegraphics[width=\imagewidthcuration,height=.21\textwidth]{figures/curation/2/175.jpg}
    \\
        Step 100
       &
        Step 125
        &
        Step 150
        &
        Step 175
\end{tabular}%
  \caption{An example of image-level curation. The image was created with VQGAN-CLIP \cite{VQGANCLIP} with the
  prompt ``ufo landing, fantastic, on Vellum, trending on /r/art.''
  The image slowly emerged from the initial random noise used to seed the GAN (step 0). After 100 steps, unwanted details started to emerge and the author aborted the process after 175 steps.
  The author then selected step 50 as ``best'' (i.e.,  most interesting and artistic) image in the batch.
  }%
  \Description{A demonstration of image-level curation. Several images generated with a text-to-image synthesis system are depicted. It is explained that one of the intermediate steps was chosen as final image.}%
  \label{fig:imagecuration}%
\end{figure*}%
%TC:endignore


==> MindTrek22 Creativity of Text-to-Image Generation/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> MindTrek22 Creativity of Text-to-Image Generation/figures/emojis/grinning-face.tex <==
😀

==> MindTrek22 Creativity of Text-to-Image Generation/figures/emojis/smiling-face-with-heart-eyes.tex <==
😍

==> figures/emojis/grinning-face.tex <==
😀

==> figures/emojis/smiling-face-with-heart-eyes.tex <==
😍
